P versus B: P Systems as a Formal Framework for Controllability of Boolean Networks

Membrane computing and P systems are a paradigm of massively parallel natural computing introduced by Gheorghe P\u{a}un in 1999, inspired by the structure of the living cell and by its biochemical reactions. In spite of this explicit biological motivation, P systems have not been extensively used in modelling real-world systems. To confirm this intuition, we establish a state of the art investigation comparing the use of P systems to that of Boolean networks in this line of research. We then propose to use P systems as a tool for setting up formal frameworks to reason about other formalisms, and we introduce Boolean P systems, specifically tailored for capturing sequential controllability of Boolean networks. We show how to tackle some technical challenges and prove that sequential controllability properly embeds in the framework of Boolean P systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{28}
\providecommand{\publicationstatus}{H. Bordihn, G. Horv\'ath, G. Vaszil (Eds.): 12th International Workshop on\\Non-Classical Models of Automata and Applications (NCMA 2022)\\
EPTCS 367, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.367.3}{10.4204/EPTCS.367.3}}
\pdfoutput=1

